Random Spatial Network Models with Core-Periphery Structure

Core-periphery structure is a common property of complex networks, which is a composition of tightly connected groups of core vertices and sparsely connected periphery vertices. This structure frequently emerges in traffic systems, biology, and social networks via underlying spatial positioning of the vertices. While core-periphery structure is ubiquitous, there have been limited attempts at modeling network data with this structure. Here, we develop a generative, random network model with core-periphery structure that jointly accounts for topological and spatial information by "core scores" of vertices. Our model achieves substantially higher likelihood than existing generative models of core-periphery structure, and we demonstrate how the core scores can be used in downstream data mining tasks, such as predicting airline traffic and classifying fungal networks. We also develop nearly linear time algorithms for learning model parameters and network sampling by using a method akin to the fast multipole method, a technique traditional to computational physics, which allow us to scale to networks with millions of vertices with minor tradeoffs in accuracy.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE = acmart
 
SAMPLES = main.tex


PDF = ${SAMPLES:%.tex=%.pdf}

all: ${PDF}


%.pdf:  %.dtx  $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

%.cls:  %.ins %.dtx
	pdflatex $<

%.pdf:  %.tex  paper/*.tex  $(PACKAGE).cls  ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM) *.pdf *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	*.synctex.gz \
	figs/*-eps-converted-to.pdf

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf sample-*.pdf *.cls *.bst


==> paper/abstract_arxiv.tex <==
\begin{abstract}
The core-periphery structure, which decompose a network into a dense core and a sparsely-connected periphery, constantly emerges from spatial networks such as traffic, biology and social networks.
%
In this paper, we propose a random network model for spatial network with core-periphery structure, which is inspired by the Kleinberg small world model.
%
In this model, we use a vertex core score to indicate the ``coreness'' of each vertex, and we randomly connect each pair of vertices with a logistic probability parameterized by their distance and core scores.
%
We compute the optimal vertex core scores in a network by fitting it to our model using a maximum likelihood estimation.
%
Results in real-world networks indicate that the fitted vertex core scores are informative machine learning features for vertex metadata prediction and network classification.
%
Furthermore, we develop near linear-time algorithms for network generation and model inference by using the fast multipole method, which allow us to scale to networks with millions of vertices with minor tradeoffs in accuracy.
\end{abstract}

